Panchromatic (Sub)millimeter Polarization Observations of HL Tau Unveil Aligned Scattering Grains

Polarization is a unique tool to study the properties of dust grains of protoplanetary disks and detail the initial conditions of planet formation. Polarization around HL Tau was previously imaged using the Atacama Large Millimeter/submillimeter Array (ALMA) at Bands 3 (3.1 mm), 6 (1.3 mm), and 7 (0.87 mm), showing that the polarization orientation changes across wavelength $\lambda$. The polarization morphology at Band 7 is predominantly parallel to the disk minor axis but appears azimuthally oriented at Band 3, with the morphology at Band 6 in between the two. We present new ~0.2" (29 au) polarization observations at Q-Band (7.0 mm) using the Karl G. Jansky Very Large Array (VLA) and at Bands 4 (2.1 mm), 5 (1.5 mm), and 7 using ALMA, consolidating HL Tau's position as the protoplanetary disk with the most complete wavelength coverage in dust polarization. The polarization patterns at Bands 4 and 5 continue to follow the morphological transition with wavelength previously identified in Bands 3, 6, and 7. Based on the azimuthal variation, we decompose the polarization into contributions from scattering ($s$) and thermal emission ($t$). We find that $s$ decreases slowly with increasing $\lambda$, and $t$ increases more rapidly with $\lambda$ which are expected from optical depth effects of toroidally aligned, scattering prolate grains. The relatively weak $\lambda$ dependence of $s$ is consistent with large, porous grains. The sparse polarization detections from the Q-band image are also consistent with toroidally aligned prolate grains.

==> deleted_content.tex <==
\subsection{Folding the Q-Band Data}

there are only a few increased points along the minor axis.... the center is unreliable because folding doesn't increase points for the center... note that the noise level depends on the location of the when folding. The noise level of the center is the same. The noise level along the major and minor axis should decrease only by a factor of sqrt(2). The noise level elsewhere will decrease by a factor of 2. 

As seen in Fig.~\ref{fig:complete_wcs}, the polarized intensity of the Q-Band image is marginally undetected at 3~$\sigma$. In this section, we utilize two symmetries to increase the signal-to-noise. If we assumed that the disk is axisymmetric and the alignment direction of the prolate grains is completely toroidal, then the resulting image is mirror symmetric with the disk minor axis as the line of symmetry (i.e., the left- and right-side of the images in Fig.~\ref{fig:obs_stokes_principal} are mirror symmetric). For Stokes~$U'$, the two halves differ by a negative sign. If we further assume that the disk is geometrically thin, then the image is also mirror symmetric with the disk major axis as the line of symmetry (i.e., the top- and bottom-half of the images in Fig~\ref{fig:obs_stokes_principal} are mirror symmetric). Again, for Stokes~$U'$, the two halves also differ by a negative sign. We can thus average Stokes~$I$, $Q'$, and $U'$ across the disk major and minor axes (with the appropriate sign change) and we are left with one quadrant of independent measurement(?). The process is analogous to folding a piece of paper in daily life and we simply use the term ``folded" as the adjective to describe the process. Assuming the noise levels are independent, folding the image effectively increases the signal-to-noise by a factor of 2 (as demonstrated in \citealt{Lin2022}). 

Folding the image is preferred over convolving the image, which is often used to increase the signal-to-noise, because beam averaging can average out the signal of polarization with different polarization directions. 


Fig... shows the Q-Band data after folding. For better visualization and comparison, we copy the single quadrant back to four quadrants with the appropriate sign change for Stokes~$U'$. 
The folded Stokes~$Q'$ image thus has ... at ... level, while the folded Stokes~$U'$ has ... detection

The folded Stokes~$Q'$ is largely positive and distributed along the disk minor axis, while the folded Stokes~$U'$ is negative in the first quadrant (top right quadrant). The results follows the consistent trend from the ALMA Bands that the positive Stokes~$Q'$ becomes more prominent. 

The results can be explained by toroidally aligned grains in the optically thin limit (Yang+2019, Mori+2021, Lin+2022). Toroidal
the center is due to beam averaging 
The complete multiwavelength trend was predicted in \cite{Lin2022}. 

We note that the averaging process would be more ideal in the $uv$-plane as opposed to the image plane. The noise in the image plane is correlated
native noise is in the $uv$-plane
Further development of the folding technique would be beneficial to clarify the level of detection and characterization of the polarization directions. 


% decomposition
As a consistency check, we show $q'$ along the major and minor axes with their decomposed $s$ and $t_{p}$ components in Fig.~\ref{fig:st_decompose}. While the scattering component is kept constant, $q'_{t}$ is equal to $t \cos^{2} i$ along the major axis and $-t$ along the minor axis from Eq.~(\ref{eq:thermal_qu_principal_frame}). 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/st_decompose.pdf}
    \caption{Caption}
    \label{fig:st_decompose}
\end{figure}
